Microlensing and the Stellar Mass Function

Traditional approaches to measuring the stellar mass function (MF) are fundamentally limited because objects are detected based on their luminosity, not their mass. These methods are thereby restricted to luminous and relatively nearby stellar populations. Gravitational microlensing promises to revolutionize our understanding of the MF. It is already technologically feasible to measure the MFs of the Galactic disk and Galactic bulge as functions of position, although the actual execution of this program requires aggressive ground-based observations including infrared interferometry, as well as the launching of a small satellite telescope. Rapid developments in microlensing, including the new technique of ``pixel lensing'' of unresolved stars, will allow one to probe the MF and luminosity function of nearby galaxies. Such observations of M31 are already underway, and pixel-lensing observations of M87 with the {\it Hubble Space Telescope} would permit detection of dark intra-cluster objects in Virgo. Microlensing techniques can also be applied to investigate the star-formation history of the universe and to search for planets with masses as small as the Earth's. Based on an invited talk at the January 1996 AAS meeting in San Antonio. PASP (June 1996) in press, (c) ASP, reproduced with permission.

==> maggieref.tex <==
\catcode`\@=11 
\def\r@fitem#1{\par \hangafter=1 \hangindent=\refindent 
\Textindent{#1}}
\def\refitem#1{\r@fitem{#1}}
\def\R@FWRITE#1{\ifreferenceopen \else \gl@bal\referenceopentrue
     \immediate\openout\referencewrite=\jobname.refs
     \toks@={\begingroup \refoutspecials \catcode`\^^M=10 }%
     \immediate\write\referencewrite{\the\toks@}\fi
    \immediate\write\referencewrite{\noexpand\refitem %
                                    {}}%
    \p@rse@ndwrite \referencewrite #1}
\catcode`\@=12 

